Unaligned Supervision For Automatic Music Transcription in The Wild

Multi-instrument Automatic Music Transcription (AMT), or the decoding of a musical recording into semantic musical content, is one of the holy grails of Music Information Retrieval. Current AMT approaches are restricted to piano and (some) guitar recordings, due to difficult data collection. In order to overcome data collection barriers, previous AMT approaches attempt to employ musical scores in the form of a digitized version of the same song or piece. The scores are typically aligned using audio features and strenuous human intervention to generate training labels. We introduce NoteEM, a method for simultaneously training a transcriber and aligning the scores to their corresponding performances, in a fully-automated process. Using this unaligned supervision scheme, complemented by pseudo-labels and pitch-shift augmentation, our method enables training on in-the-wild recordings with unprecedented accuracy and instrumental variety. Using only synthetic data and unaligned supervision, we report SOTA note-level accuracy of the MAPS dataset, and large favorable margins on cross-dataset evaluations. We also demonstrate robustness and ease of use; we report comparable results when training on a small, easily obtainable, self-collected dataset, and we propose alternative labeling to the MusicNet dataset, which we show to be more accurate. Our project page is available at https://benadar293.github.io

==> tables/table_em_guitar.tex <==
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Test Set & \multicolumn{6}{|c|}{GuitarSet} \\
\hline
Transcription Level & \multicolumn{3}{|c|}{Note} & \multicolumn{3}{|c|}{Frame} \\
\hline
 & P & R & F1 & P & R & F1 \\
\hline
% Synth & 86.0 & 82.1 & 83.8 & 79.1 & 72.6 & 74.7 & 79.5 & 79.3 & 79.1 & 66.3 & 78.6 & 71.0 \\
Single Labeling & 83.3 & 78.6 & 80. & 82.0 & 80.5 & 80.9 \\
\hline
\end{tabular}
\end{center}
\caption{Effect of EM guitarset}\label{table:em_guitar}

==> tables/table_musicnet.tex <==
\caption{Transcription results on MusicNet test set. We don't test on solo piano pieces from the test set (1759, 2303, 2556) since MAPS and MAESTRO are more reliable. We provide results for string and wind separately. In the table we use the same test split as in~\cite{DBLP:conf/mm/CheukHS21}. The string test set includes piece 2628 which contains strings and piano. The results on the pieces with only strings (2106, 2298, 2382) are 78.1, 69.8 note- and frame- F1 respectively using our test annotation, and 61.0, 67.0 note- and frame- F1 respectively using the original test annotation. First column - train set. MusicNet$_{EM}$ is the MusicNet recordings with our annotation. Columns 2-9 - MusicNet test set with with our annotation, columns 10-15 - MusicNet test set with original annotation. We also report the distance computed by DTW between prediction and the unaligned midi of the test set (lower is better, normalized by target midi length in frames). For the test set, we compute DTW for onsets and for frames separately. Unsurprisingly, there is a correlation between F1 score and DTW distance. We believe that DTW distance between prediction and unaligned midi can be used as an additional metric for evaluation in the absence of precise annotation. We also compare against~\cite{DBLP:journals/corr/abs-2111-03017}, which was trained on a different split. Still, the difference is significant.
% As can be seen, our method performs better than both the synthetic data pre-trained model, and the model trained with the original annotation of MusicNet, and surpasses~\cite{DBLP:conf/mm/CheukHS21} in almost all metrics. 
% Similar to Table~\ref{transcription_table}, further training of the model trained on synthetic data with the original MusicNet annotation significantly degrades performance.
}\label{table:musicnet_combined}

\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
& \multicolumn{4}{|c|}{Note} & \multicolumn{4}{|c|}{Frame} & \multicolumn{3}{|c|}{Note} & \multicolumn{3}{|c|}{Frame} \\
\hline
& P & R & F1 & dtw & P & R & F1 & dtw & P & R & F1 & P & R & F1 \\
\hline
% & \multicolumn{8}{|c|}{MusicNet$_{EM}$ test} & \multicolumn{6}{|c|}{MusicNet test} \\
% \hline
% & \multicolumn{4}{|c|}{Note} & \multicolumn{4}{|c|}{Frame} & \multicolumn{3}{|c|}{Note} & \multicolumn{3}{|c|}{Frame} \\
% \hline
% Train Set & P & R & F1 & dtw & P & R & F1 & dtw & P & R & F1 & P & R & F1 \\
% \hline
% All test set with piano:
% Synth & 80.3 & 72.1 & 75.6 & 0.26 & 76.2 & 58.8 & 65.5 & 1.36 & 60.8 & 54.1 & 56.8 & 71.5 & 55.3 & 61.2 \\
% \hline
% MusicNet orig. & 55.7 & 44.2 & 48.3 & 0.86 & 66.2 & 61.1 & 61.4 & 1.18 & 51.5 & 40.1 & 44.2 & 71.8 & 63.4 & 65.2 \\
% \hline
% MusicNet$_{EM}$ & 83.9 & 87.4 & \textbf{85.6} & \textbf{0.16} & 72.7 & 78.6 & \textbf{75.4} & \textbf{0.93} & 67.0 & 65.6 & 66.1 & 72.5 & 73.5 & \textbf{72.6} \\
% \hline
% SC & 84.3 & 83.4 & 83.7 & 0.19 & 77.4 & 71.2 & 73.9 & 1.02 & 68.1& 66.2 & \textbf{66.9} & 73.7 & 67.8 & 70.2 \\
% \hline
% % This is the 3 only-string pieces:
% & \multicolumn{8}{|c|}{MusicNet$_{EM}$ \textbf{Strings} test 2106, 2298, 2382} & \multicolumn{6}{|c|}{MusicNet String test} \\
% \hline
% & \multicolumn{4}{|c|}{Note} & \multicolumn{4}{|c|}{Frame} & \multicolumn{3}{|c|}{Note} & \multicolumn{3}{|c|}{Frame} \\
% \hline
% Train Set & P & R & F1 & dtw & P & R & F1 & dtw & P & R & F1 & P & R & F1 \\
% \hline
% MusicNet orig. & 23.8 & 22.4 & 23.1 & 0.99 & 55.6 & 65.8 & 60.1 & 1.03 & 42.2 & 34.6 & 37.5 & 66.1 & \textbf{71.7} & \textbf{68.5} \\
% \hline
% Synth & 71.4 & 60.0 & 64.6 & 0.32 & 70.1 & 43.1 & 52.4 & 1.40 & 53.8 & 42.3 & 46.4 & 66.3 & 37.7 & 47.1 \\
% MusicNet$_{EM}$ (ours) & \textbf{80.4} & \textbf{76.5} & \textbf{78.1} & \textbf{0.21} & \textbf{72.2} & \textbf{67.8} & \textbf{69.8} & \textbf{0.87} & \textbf{66.8} & \textbf{57.6} & \textbf{61.0} & \textbf{72.3} & 62.7 & 67.0 \\
% \hline
% This has also one piano+violin:
& \multicolumn{8}{|c|}{MusicNet$_{EM}$ \textbf{Strings} test 2106, 2298, 2382, 2628} & \multicolumn{6}{|c|}{Original Test Annotation} \\
\hline
~\cite{DBLP:conf/mm/CheukHS21} &&&&&&&&& 63.6 & 58.8 & 61.0 & \textbf{78.9} & 60.7 & 68.4 \\
\hline
MusicNet orig. & 36.0 & 33.3 & 34.6 & 1.02 & 58.5 & 69.4 & 63.4 & 1.14 & 44.1 & 37.1 & 39.9 & 66.2 & \textbf{73.5} & \textbf{69.4} \\
\hline
Synth & 73.0 & 59.7 & 65.2 & 0.32 & 70.3 & 45.5 & 54.4 & 1.51 & 57.3 & 44.2 & 49.1 & 66.7 & 40.9 & 49.8 \\
MusicNet$_{EM}$ (ours) & \textbf{81.8} & \textbf{78.7} & \textbf{80.0} & \textbf{0.21} & \textbf{73.2} & \textbf{69.8} & \textbf{71.3} & \textbf{0.97} & \textbf{68.6} & \textbf{61.1} & \textbf{63.9} & 72.4 & 65.0 & 68.3 \\
\hline
& \multicolumn{8}{|c|}{MusicNet$_{EM}$ \textbf{Wind} test 1819, 2416} & \multicolumn{6}{|c|}{Original Test Annotation} \\
\hline
% & \multicolumn{4}{|c|}{Note} & \multicolumn{4}{|c|}{Frame} & \multicolumn{3}{|c|}{Note} & \multicolumn{3}{|c|}{Frame} \\
% \hline
% Train Set & P & R & F1 & dtw & P & R & F1 & dtw & P & R & F1 & P & R & F1 \\
% \hline
~\cite{DBLP:conf/mm/CheukHS21} & &&&&&&&& 48.6 & 47.9 & 48.2 & 69.8 & 65.8 & 67.4
\\
\hline
MusicNet orig. & 50.3 & 46.6 & 48.4 & 0.79 & 66.8 & 75.0 & 70.5 & 1.18 & 40.0 & 36.3 & 38.0 & 69.9 & 78.3 & 73.4 \\
\hline
Synth & 80.4 & 77.2 & 78.8 & 0.26 & \textbf{72.7} & 59.3 & 65.3 & 1.47 & 56.8 & 54.0 & 55.4 & \textbf{71.8} & 58.5 & 64.3 \\
MusicNet$_{EM}$ & \textbf{84.2} & \textbf{91.1} & \textbf{87.5} & \textbf{0.17} & 71.4 & \textbf{79.0} & \textbf{75.0} & \textbf{1.01} & \textbf{58.9} & \textbf{63.1} & \textbf{60.9} & 70.7 & \textbf{78.2} & \textbf{74.2} \\
% 48.6 & 47.9 & 48.2 & 69.8 & 65.8 & 67.4
\hline
& \multicolumn{8}{|c|}{} & \multicolumn{6}{|c|}{~\cite{DBLP:journals/corr/abs-2111-03017} test split} \\
\hline
% & \multicolumn{4}{|c|}{Note} & \multicolumn{4}{|c|}{Frame} & \multicolumn{3}{|c|}{Note} & \multicolumn{3}{|c|}{Frame} \\
% \hline
% Train Set & P & R & F1 & dtw & P & R & F1 & dtw & P & R & F1 & P & R & F1 \\
% \hline
% MusicNet orig. &&&&&&&&& 43.1 & 38.4 & 40.4 & 68.8 & 77.7 & 72.8 \\
% Synth. &&&&&&&&& 60.8 & 54.1 & 56.8 & 71.5 & 55.3 & 61.2 \\
% MusicNet+ &&&&&&&&& 67.2 & 64.7 & 65.6 & 73.6 & 72.7 & 72.7 \\
% \hline
~\cite{DBLP:journals/corr/abs-2111-03017} &\multicolumn{8}{|c|}{} &&& 50.0 & & & 68.0 \\
\hline
\end{tabular}
\end{center}
% \caption{Transcription results on MusicNet test set. First column - train set. MusicNet+ is the MusicNet recordings with our annotation, and SC is the self collected data. Columns 2-9 - MusicNet test with with our annotation, columns 10-15 - MusicNet test set with original annotation. We also report the distance computed by DTW between prediction and the separate-source midi of the test set (lower is better, normalized by target midi length). For the test set, we compute DTW for onsets and for frames separately. Unsurprisingly, there is a correlation between F1 score and DTW distance. We believe that DTW distance between prediction and separate-source midi can be used as a metric for evaluation in the absence of precise annotation. As can be seen, our method performs better than both the synthetic data pre-trained model, and the model trained with the original annotation of MusicNet. Similar to Table~\ref{transcription_table}, further training of the model trained on synthetic data with the original MusicNet annotation significantly degrades performance.}\label{table:musicnet_combined}



% \begin{center}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% Test Set & \multicolumn{6}{|c|}{MusicNet} \\
% \hline
% Level & \multicolumn{3}{|c|}{Note} & \multicolumn{3}{|c|}{Frame} \\
% \hline
%  & P & R & F1 & P & R & F1 \\
% \hline
% MusicNet & 51.5 & 40.1 & 44.2 & 71.8 & 63.4 & 65.2 \\
% \hline
% Synth & 60.8 & 54.1 & 56.8 & 71.5 & 55.3 & 61.2 \\
% \hline
% MusicNet (ours) & 67.0 & 65.6 & 66.1 & 72.5 & 73.5 & 72.6 \\
% \hline
% Ours & 68.1& 66.2 & 66.9 & 73.7 & 67.8 & 70.2 \\
% % Ours (Weakly supervised) & 94.1 & 87.3 & 90.5 & 72.8 & 77.0 & 73.6 & 87.3 & 85.9 & \textbf{86.6} & 58.1 & 88.5 & 68.8 \\
% \hline
% \end{tabular}
% \end{center}
% \caption{Transcription results on MusicNet using original test annotation}\label{musicnet_table}

==> tables/table_musicnet_em_instruments.tex <==
\caption{Instrument-sensitive Transcription results (note-with-instrument). 
%A note is considered correct only if its predicted instrument is correct. 
We show results on the MusicNet test set, and our proposed labels -- MusicNet$_{EM}$. We also compare to~\citet{DBLP:journals/taslp/WuC020} who evaluate on the MusicNet test set.
%~\citet{DBLP:journals/corr/abs-2111-03017} only show note+offset+instrument (not note+instrument) on a different split, where they report $34\%$. Based on Tables~\ref{transcription_table},~\ref{table:musicnet_combined},~\ref{guitarset_table} it seems that a large portion of the errors is not in the model, but rather in the original labels.  
Notice the improvements for horn, bassoon, and clarinet. %compared to~\cite{DBLP:journals/taslp/WuC020}, even when using the original MusicNet annotation. 
For Violin, Cello, and Viola, accuracy according to the original annotation is comparable. 
%\textbf{However, we believe the original annotation does not reflect real performance}. For example, if the model onset timing detection is correct and the annotation's onset timing is incorrect (which we believe to happen often), this will reduce both precision and recall. \textbf{
However, this is probably due to label quality. See Supplementary material for more detail and a qualitative comparison.
%,  to~\cite{DBLP:journals/taslp/WuC020} that clearly demonstrates the better performance of our approach. 
% Note that we do not require threshold optimization, contrary to~\cite{DBLP:journals/taslp/WuC020}. 
We also evaluate this task on MAPS, MAESTRO, and GuitarSet. %Metrics are lower than Tables~\ref{transcription_table},~\ref{table:musicnet_combined},~\ref{guitarset_table} since this is a harder task. On piano and guitar there are few mistakes in instrument, as the metrics are close to the ones in Tables~\ref{transcription_table},~\ref{guitarset_table}. 
The most challenging instrument is viola, due to the resemblance to both violin and cello, hampering instrument identification accuracy. }\label{table:musicnet_em_by_instrument}
\begin{center}
\begin{tabular}{|c|c|}
\hline
%  & \multicolumn{3}{|c|}{Ours ZS} & \multicolumn{3}{|c|}{~\cite{DBLP:journals/corr/abs-2111-03017} ZS} & \multicolumn{3}{|c|}{~\cite{DBLP:journals/corr/abs-2111-03017}} \\
% \hline
% Instrument & P & R & F1 & P & R & F1 & P & R & F1 \\
% \hline
%  & \multicolumn{3}{|c|}{Ours, orig. labels} & &  \\
% \hline
% Instrument & P & R & F1 \\
% \hline
% piano (pn), violin (vn), viola (va), cello (vc), flute (fl),
% horn (hn), bassoon (bn), clarinet (cl), harpsichord (hpd), contrabass (db), and oboe (ob)
% Piano (1759, 2303, 2556, 2628) & 88.4 & 87.4 & 87.9 & 70.9 & 70.9 & 70.9 & 74.6 & 64.7 & 68.9 \\
% \hline
test instrument & note-with-inst. F1 \\
\hline
Violin & 87.3 \\
Viola &	61.1 \\
Cello &	79.9 \\
Bassoon & 78.0 \\
Clarinet & 86.8 \\
Horn & 75.0 \\
\hline
\end{tabular}
\end{center}
% \caption{Instrument-sensitive Transcription results. Notice the outstanding improvement for horn, bassoon, and clarinet compared to~\cite{DBLP:journals/taslp/WuC020}, even when using the original MusicNet annotation.}\label{table:instrument_sensitive_v2}

==> tables/table_musicnet_v2.tex <==
\caption{Transcription results on MusicNet test set, reported for string and wind instruments separately. In the table we use the same test split as \citet{DBLP:conf/mm/CheukHS21} (excluding piano pieces, which are less reliable compared to MAPS and MAESTRO). 
%which is \textbf{string instruments}: pieces 2106, 2298, 2382, 2628 and \textbf{wind instruments}: pieces 1819, 2416. We don't test on solo piano pieces from the test set (1759, 2303, 2556) since MAPS and MAESTRO are more reliable. The string test set includes piece 2628 which contains strings and piano. 
%The results on the pieces with only strings (2106, 2298, 2382) are 78.1, 69.8 note- and frame- F1 respectively using our test annotation, and 61.0, 67.0 note- and frame- F1 respectively using the original test annotation. 
Results compare the same training on three different datasets (rows), evaluated on both the given MusicNet annotations, and the ones generated using our unaligned supervision scheme (columns). 
We also report the distance computed by DTW between frame prediction and the frame activation in the unaligned MIDI of the test set (lower is better, normalized by target midi length in frames)\abc{I don't understand the DTW score thing}. Note-level DTW can be found in the Supplementary, where we show a correlation between F1 score and DTW distance. 
%We believe that DTW distance between prediction and unaligned midi can be used as an additional metric for evaluation in the absence of precise annotation.  --- remember to add this to the text
We also compare against \citet{DBLP:journals/corr/abs-2111-03017}, which use a different split. 
%Still, the difference is significant.
}\label{table:musicnet_combined}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
& \multicolumn{3}{|c|}{Note} & \multicolumn{3}{|c|}{Frame} & \multicolumn{3}{|c|}{Note} & \multicolumn{4}{|c|}{Frame} \\
\hline
& P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & DTW \\
\hline
& \multicolumn{6}{|c|}{MusicNet$_{EM}$ \textbf{Strings} test} & \multicolumn{7}{|c|}{MusicNet \textbf{Strings} test} \\
\hline
~\cite{DBLP:conf/mm/CheukHS21} &&&&&&& 63.6 & 58.8 & 61.0 & \textbf{78.9} & 60.7 & 68.4 & - \\
\hline
MusicNet & 36.0 & 33.3 & 34.6 & 58.5 & 69.4 & 63.4 & 44.1 & 37.1 & 39.9 & 66.2 & \textbf{73.5} & \textbf{69.4} & 1.14 \\
\hline
Synth & 73.0 & 59.7 & 65.2 & 70.3 & 45.5 & 54.4 & 57.3 & 44.2 & 49.1 & 66.7 & 40.9 & 49.8 & 1.51 \\
MusicNet$_{EM}$ (ours) & \textbf{81.8} & \textbf{78.7} & \textbf{80.0} & \textbf{73.2} & \textbf{69.8} & \textbf{71.3} & \textbf{68.6} & \textbf{61.1} & \textbf{63.9} & 72.4 & 65.0 & 68.3 & \textbf{0.97}\\
\hline
& \multicolumn{6}{|c|}{MusicNet$_{EM}$ \textbf{Wind} test} & \multicolumn{7}{|c|}{MusicNet \textbf{Wind} test} \\
\hline
~\cite{DBLP:conf/mm/CheukHS21} & &&&&&& 48.6 & 47.9 & 48.2 & 69.8 & 65.8 & 67.4 & -
\\
\hline
MusicNet & 50.3 & 46.6 & 48.4 & 66.8 & 75.0 & 70. & 40.0 & 36.3 & 38.0 & 69.9 & 78.3 & 73.4 & 1.18 \\
\hline
Synth & 80.4 & 77.2 & 78.8 & \textbf{72.7} & 59.3 & 65.3 & 56.8 & 54.0 & 55.4 & \textbf{71.8} & 58.5 & 64.3 & 1.47 \\
MusicNet$_{EM}$ & \textbf{84.2} & \textbf{91.1} & \textbf{87.5} & 71.4 & \textbf{79.0} & \textbf{75.0} & \textbf{58.9} & \textbf{63.1} & \textbf{60.9} & 70.7 & \textbf{78.2} & \textbf{74.2} & \textbf{1.01}\\
\hline
& \multicolumn{6}{|c|}{} & \multicolumn{7}{|c|}{~\cite{DBLP:journals/corr/abs-2111-03017} test split} \\
\hline
~\cite{DBLP:journals/corr/abs-2111-03017} &\multicolumn{6}{|c|}{} &- & - & 50.0 & - & - & 68.0 & - \\
\hline
\end{tabular}
\end{center}

==> tables/table_note_with_instrument_musicnet_em.tex <==
\caption{Instrument-sensitive Transcription results (note-with-instrument). 
%A note is considered correct only if its predicted instrument is correct. 
We show results on the MusicNet test set, and our proposed labels -- MusicNet$_{EM}$. We also compare to~\citet{DBLP:journals/taslp/WuC020} who evaluate on the MusicNet test set.
%~\citet{DBLP:journals/corr/abs-2111-03017} only show note+offset+instrument (not note+instrument) on a different split, where they report $34\%$. Based on Tables~\ref{transcription_table},~\ref{table:musicnet_combined},~\ref{guitarset_table} it seems that a large portion of the errors is not in the model, but rather in the original labels.  
Notice the improvements for horn, bassoon, and clarinet. %compared to~\cite{DBLP:journals/taslp/WuC020}, even when using the original MusicNet annotation. 
For Violin, Cello, and Viola, accuracy according to the original annotation is comparable. 
%\textbf{However, we believe the original annotation does not reflect real performance}. For example, if the model onset timing detection is correct and the annotation's onset timing is incorrect (which we believe to happen often), this will reduce both precision and recall. \textbf{
However, this is probably due to label quality. See Supplementary material for more detail and a qualitative comparison.
%,  to~\cite{DBLP:journals/taslp/WuC020} that clearly demonstrates the better performance of our approach. 
% Note that we do not require threshold optimization, contrary to~\cite{DBLP:journals/taslp/WuC020}. 
We also evaluate this task on MAPS, MAESTRO, and GuitarSet. %Metrics are lower than Tables~\ref{transcription_table},~\ref{table:musicnet_combined},~\ref{guitarset_table} since this is a harder task. On piano and guitar there are few mistakes in instrument, as the metrics are close to the ones in Tables~\ref{transcription_table},~\ref{guitarset_table}. 
The most challenging instrument is viola, due to the resemblance to both violin and cello, hampering instrument identification accuracy. }\label{table:instrument_sensitive_em}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
%  & \multicolumn{3}{|c|}{Ours ZS} & \multicolumn{3}{|c|}{~\cite{DBLP:journals/corr/abs-2111-03017} ZS} & \multicolumn{3}{|c|}{~\cite{DBLP:journals/corr/abs-2111-03017}} \\
% \hline
% Instrument & P & R & F1 & P & R & F1 & P & R & F1 \\
% \hline
%  & \multicolumn{3}{|c|}{Ours, orig. labels} & &  \\
% \hline
% Instrument & P & R & F1 \\
% \hline
% piano (pn), violin (vn), viola (va), cello (vc), flute (fl),
% horn (hn), bassoon (bn), clarinet (cl), harpsichord (hpd), contrabass (db), and oboe (ob)
% Piano (1759, 2303, 2556, 2628) & 88.4 & 87.4 & 87.9 & 70.9 & 70.9 & 70.9 & 74.6 & 64.7 & 68.9 \\
% \hline
& note F1 & note-with-inst. F1 & frame F1 &	note-with-offset F1 \\
\hline
% MAPS & 82.0 & 82.0 & 69.1 & 37.7 \\
% MAESTRO	& 85.0 & 85.0 & 65.2 & 31.9 \\
% GuitarSet &	72.8 & - & 68.4 & 30.7 \\
MusicNetEM	& 91.4 & 88.1 & 82.5 & 71.4 \\
MusicNetEM wind & 88.5 & 79.9 &	83.1 & 65.0 \\ 
MusicNetEM strings & 89.1 & 85.5 & 82.6 & 77.7 \\
MusicNetEM strings*	& 85.9 & 81.1 &	79.0 & 75.1 \\
\hline
\end{tabular}
\end{center}
% \caption{Instrument-sensitive Transcription results. Notice the outstanding improvement for horn, bassoon, and clarinet compared to~\cite{DBLP:journals/taslp/WuC020}, even when using the original MusicNet annotation.}\label{table:instrument_sensitive_v2}

==> tables/table_note_with_instrument_v2.tex <==
\caption{Instrument-sensitive Transcription results. Notice the outstanding improvement for horn, bassoon, and clarinet compared to~\cite{DBLP:journals/taslp/WuC020}, even when using the original MusicNet annotation.}\label{table:instrument_sensitive_v2}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
 & \multicolumn{3}{|c|}{Note+Instr.} &  \multicolumn{3}{|c|}{Note} & \multicolumn{3}{|c|}{Frame} \\
\hline
Instrument & P & R & F1 & P & R & F1 & P & R & F1 \\
\hline
Piano (MAPS)  & 87.7& 82.9 & 85.1 & 87.7& 82.9 & 85.1 & 83.9 & 62.2 & 70.6 \\
Piano (MAESTRO)  & 94.1 & 81.4 & 86.9 & 94.1 & 81.4 & 86.9 & 79.7 & 59.2 & 66.7 \\

% note precision                : 0.927 ± 0.067
%                             note recall                   : 0.781 ± 0.141
%                             note f1                       : 0.841 ± 0.101
%                             note overlap                  : 0.531 ± 0.152
%               note-with-offsets precision                : 0.281 ± 0.189
%               note-with-offsets recall                   : 0.251 ± 0.186
%               note-with-offsets f1                       : 0.264 ± 0.187
%               note-with-offsets overlap                  : 0.871 ± 0.058
%             note-with-instrument precision                : 0.924 ± 0.077
%             note-with-instrument recall                   : 0.778 ± 0.144
%             note-with-instrument f1                       : 0.838 ± 0.108
%             note-with-instrument overlap                  : 0.531 ± 0.152
%               note-with-velocity precision                : 0.927 ± 0.067
%               note-with-velocity recall                   : 0.781 ± 0.141
%               note-with-velocity f1                       : 0.841 ± 0.101
%               note-with-velocity overlap                  : 0.531 ± 0.152
%   note-with-offsets-and-velocity precision                : 0.281 ± 0.189
%   note-with-offsets-and-velocity recall                   : 0.251 ± 0.186
%   note-with-offsets-and-velocity f1                       : 0.264 ± 0.187
%   note-with-offsets-and-velocity overlap                  : 0.871 ± 0.058
%                           frame f1                       : 0.705 ± 0.081
%                           frame precision                : 0.686 ± 0.115
%                           frame recall                   : 0.747 ± 0.112

Guitar (GuitarSet) & 92.4 & 77.8 & 83.8 & 92.7 & 78.1 & 84.1 & 68.6 & 74.7 & 70.5 \\
Violin (2106, 2382, 2628) &  \\
Viola (2106, 2382) &  \\
Cello (2106, 2298, 2382) &  \\
Horn (1819, 2416) & \\
Bassoon (1819, 2416) &  \\
Clarinet (1819, 2416) &  \\
% Harpsichord & && &&&&&& \\
\hline
\end{tabular}
\end{center}
% \caption{Instrument-sensitive Transcription results. Notice the outstanding improvement for horn, bassoon, and clarinet compared to~\cite{DBLP:journals/taslp/WuC020}, even when using the original MusicNet annotation.}\label{table:instrument_sensitive_v2}

==> tables/table_pitch_shift_guitar.tex <==
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 & \multicolumn{6}{|c|}{GuitarSet} \\
\hline
& \multicolumn{3}{|c|}{Note} & \multicolumn{3}{|c|}{Frame} \\
\hline
 & P & R & F1 & P & R & F1 \\
\hline
MusicNet$_{EM}$ w/o pitch shift & 71.1 & 81.2 & 75.4 & 73.1 & 84.1 & 77.8 \\
\hline
MusicNet$_{EM}$ w/ pitch shift & 86.6 & 80.4 & 82.9 & 79.3 & 84.8 & 81.6 \\
\hline
\end{tabular}
\end{center}
\caption{Effect of pitch shift when evaluating on GuitarSet.}\label{table:pitch_shift_guitar}
